PerOS: Personalized Self-Adapting Operating Systems in the Cloud

Operating systems (OSes) are foundational to computer systems, managing hardware resources and ensuring secure environments for diverse applications. However, despite their enduring importance, the fundamental design objectives of OSes have seen minimal evolution over decades. Traditionally prioritizing aspects like speed, memory efficiency, security, and scalability, these objectives often overlook the crucial aspect of intelligence as well as personalized user experience. The lack of intelligence becomes increasingly critical amid technological revolutions, such as the remarkable advancements in machine learning (ML). Today's personal devices, evolving into intimate companions for users, pose unique challenges for traditional OSes like Linux and iOS, especially with the emergence of specialized hardware featuring heterogeneous components. Furthermore, the rise of large language models (LLMs) in ML has introduced transformative capabilities, reshaping user interactions and software development paradigms. While existing literature predominantly focuses on leveraging ML methods for system optimization or accelerating ML workloads, there is a significant gap in addressing personalized user experiences at the OS level. To tackle this challenge, this work proposes PerOS, a personalized OS ingrained with LLM capabilities. PerOS aims to provide tailored user experiences while safeguarding privacy and personal data through declarative interfaces, self-adaptive kernels, and secure data management in a scalable cloud-centric architecture; therein lies the main research question of this work: How can we develop intelligent, secure, and scalable OSes that deliver personalized experiences to thousands of users?

==> sections/6_plan.tex <==
\newpage
\section{First-Year Plan} \label{sec:plan}

I sketch a plan below for my first-year research by means of milestones (\textbf{M}s) and deliverables (\textbf{D}s)

\begin{enumerate}[label=\textbf{M\arabic*}, ref=\textbf{M\arabic*}]
    \item \label{m1} \underline{Literature review and benchmarking existing artifacts:}
    
    I plan to spend the first three months studying related work, evaluating their artifacts if available, and collecting training data for the user-facing LLM (\S\ref{subsec:method1}).

    \textbf{(D1.1)} Literature review with benchmarking results comparing related work;
    
    \textbf{(D1.2)} Training datasets or data sources for the LLM;
    
    \item \label{m2} \underline{Start building the first prototype towards answering \ref{rq1}:}

    Over the next three months, I plan to start developing the initial prototype of \sysname{} centered around the declarative interface (\S\ref{sec:interface}). This development phase includes the training of the two-tower LLM, comprising the Interpreter and Director components, along with building the supporting infrastructure such as the Actuator and Watchdog, each developed \textit{independently} (Figure~\ref{fig:interface}).

    The primary goal is to conduct an initial evaluation of the prototype and compare its performance against the results obtained in \ref{m1}. The evaluation process will emphasize \textit{isolated} assessments of the two distinct parts (\S\ref{subsec:method1}). Ideally, these findings should be publishable as a workshop paper, allowing me to gather some initial feedback from the community (even if it is rejected).

    \textbf{(D2.1)} Minimal working prototype of \sysname{} with the declarative interface;
    
    \textbf{(D2.2)} Short paper containing the initial results and the future system blueprint (potential venues include HotOS, HotNets, or a co-held workshop at a major conference);

    \item \label{m3} \underline{Answering \ref{rq1}}:
    
    Building upon the outcomes of \ref{m2}, my goal is to finalize the development of the prototype (Figure~\ref{fig:interface}) and carry out extensive experiments within the upcoming three months. This phase will involve the integration of the two system parts, as well as the retraining policy and the actual invocation of system APIs, leading to a comprehensive evaluation.
    Simultaneously, I will be actively working on drafting a paper for a major submission, based on the feedback previously acquired. Writing will help me crystallize the storyline from the start.

    \textbf{(D3.1)} Artifact depicted in Figure~\ref{fig:interface};
    
    \textbf{(D3.2)} Submission to a major conference such as MLSys, ASPLOS, OSDI, and NSDI;

    \item \label{m4} \underline{Literature review and investigating microkernels for \ref{rq2}}:
    
    During the last three months of my first year, my plan is to transition gradually to focusing on \ref{rq2} while awaiting the submission result. Just as I did in \ref{m1}, I will initiate this phase by conducting an in-depth literature review.
    At the same time, I intend to delve deeply into microkernels and subsystems, given their pivotal role in addressing \ref{rq2}.

    \textbf{(D4)} Literature review and the choice of microkernel for \sysname{};

\end{enumerate}
